Voting-based Approaches For Differentially Private Federated Learning

Differentially Private Federated Learning (DPFL) is an emerging field with many applications. Gradient averaging based DPFL methods require costly communication rounds and hardly work with large-capacity models, due to the explicit dimension dependence in its added noise. In this work, inspired by knowledge transfer non-federated privacy learning from Papernot et al.(2017; 2018), we design two new DPFL schemes, by voting among the data labels returned from each local model, instead of averaging the gradients, which avoids the dimension dependence and significantly reduces the communication cost. Theoretically, by applying secure multi-party computation, we could exponentially amplify the (data-dependent) privacy guarantees when the margin of the voting scores are large. Extensive experiments show that our approaches significantly improve the privacy-utility trade-off over the state-of-the-arts in DPFL.

==> acknowledgement.tex <==
\section*{Acknowledgements}

\textbf{Do not} include acknowledgements in the initial version of
the paper submitted for blind review.

If a paper is accepted, the final camera-ready version can (and
probably should) include acknowledgements. In this case, please
place such acknowledgements in an unnumbered section at the
end of the paper. Typically, this will include thanks to reviewers
who gave useful comments, to colleagues who contributed to the ideas,
and to funding agencies and corporate sponsors that provided financial
support.


==> related_work.tex <==
\section{Related work}
\subsection{Gradient-based DPFL}
\textbf{Agent-level global DP}  Recent work~\cite{dp_fl, dp_language} apply differential privacy to federated learning and offer agent-level global differential privacy. These approaches require a trusted server, and noise is added to the server's aggregated model updates.

\textbf{Record-level global DP}
Record-level global DP has been widely studied in differentially private machine learning. One popular approach is to inject Gaussian noise to the clipped gradient at each step of the stochastic gradient descent (SGD). We make several modifications to extend it with the FL framework. As depicted in Figure [], each agent performs a variable number of NoisySGD updates; the model updates are averaged at the server in each communication round.  Given that the varied data size across agents may affect the privacy guarantee through subsampling, we often seek the weakest privacy guarantee (largest $\epsilon$) among agents.

%The vanilla DP-FedAvg algorithm~\ref{alg: standard_dp} only supports the agent-level global DP guarantee, where the noise is added to the sum of all scaled updates.  To satisfy the agent-level local DP, we add noise to the scaled updates instead, see algorithm~\ref{alg: agent_dp}.  Algorithm~\ref{alg: agent_dp} combined with secure multiparty computation (MPC) and algorithm~\ref{alg: standard_dp} maintains the same agent-level global DP. Moreover, algorithm~\ref{alg: agent_dp} satisfies agent-level global DP with respect to Noise scale $\cN(0, \sigma^2/m_t)$.

\subsection{Voting-based DP}

